How to Solve Fair $k$-Center in Massive Data Models

Fueled by massive data, important decision making is being automated with the help of algorithms, therefore, fairness in algorithms has become an especially important research topic. In this work, we design new streaming and distributed algorithms for the fair $k$-center problem that models fair data summarization. The streaming and distributed models of computation have an attractive feature of being able to handle massive data sets that do not fit into main memory. Our main contributions are: (a) the first distributed algorithm; which has provably constant approximation ratio and is extremely parallelizable, and (b) a two-pass streaming algorithm with a provable approximation guarantee matching the best known algorithm (which is not a streaming algorithm). Our algorithms have the advantages of being easy to implement in practice, being fast with linear running times, having very small working memory and communication, and outperforming existing algorithms on several real and synthetic data sets. To complement our distributed algorithm, we also give a hardness result for natural distributed algorithms, which holds for even the special case of $k$-center.

==> lb-proof1.tex <==
\section{Distributed $k$-Center Lower Bound}

In this section we present the formal details of the lower bound discussed in Section~4 of the main paper. 
For a natural number $n$, $[n]$ denotes the set $\{1,2,\ldots,n\}$.
%\paragraph{The Communication Model $\mathrm{PSim}$.} TODO: define the model using notation from previous sections.
\paragraph{The metric $\mathcal{M}(n')$.} 
The points in the metric space on $n = 9n'+7$ points are given by 
\[S := \{a^*,b_1^*,b_2^*,c^*,a,b,c\} \cup S_1 \cup S_2 \cup S_3,\]
where $|S_1| = |S_2| = |S_3| = 3n'$.
Note that $S_1,S_2,S_3$ are pairwise disjoint and are also disjoint from $\{a^*,b_1^*,b_2^*,c^*,a,b,c\}$. See Figure \ref{metric} for a drawing of the metric; importantly, $x$ is not a point in the metric but is only used to define the pairwise distances. 

\begin{figure}[h]
    \centering{\includegraphics[width=.4\textwidth]{metric1.pdf}}
    \caption{\footnotesize The underlying metric for $n'=2$}
    \label{metric}
\end{figure}
% \textbf{Need to mention that x is not a point in the metric space.}
The pairwise distances are given in \Cref{metric-pairwisedist}.
Note that if the table entry $i,j$ is indexed by sets, then the entry corresponds to the distance between distinct points in the sets.
\begin{table}[htp]
	\ra{1.5}
	\centering
	\adjustbox{max width = \textwidth}{
		\begin{tabular}{@{}c|ccccccccccc@{}}
			 & $a^*$ & $b_1^*$ & $b_2^*$ & $c^*$ & $a$ & $b$ & $c$  & $S_1$ & $S_2$ & $S_3$\\ 
			 \toprule
$a^*$& $0$ & $1$& $1$ &$2$ & $1$ & $2$ & $3$ & $1$ & $2$ & $3$\\
$b_1^*$ & $1$ & $0$ & $2$ &$1$ & $2$ & $1$ & $2$  & $2$ & $1$ & $2$ \\
$b_2^*$ & $1$ & $2$ &$0$ &$1$ & $2$ & $1$ & $2$ & $2$ & $1$ & $2$ \\
$c^*$ & $2$ & $1$ & $1$ &$0$ & $3$ & $2$ & $1$  & $3$ & $2$ & $1$ \\
$a$ & $1$ & $2$ & $2$ &$3$ & $0$ & $3$ & $4$  & $2$ & $3$ & $4$ \\
$b$ & $2$ & $1$ & $1$ &$2$ & $3$ & $0$ & $3$ & $3$ & $2$ & $3$ \\
$c$ & $3$ & $2$ & $2$ &$1$ & $4$ & $3$ & $0$  & $4$ & $3$ & $2$ \\
$S_1$ & $1$ & $2$ & $2$ &$3$ & $2$ & $3$ & $4$ & $2$ & $2$ & $2$ \\
$S_2$ & $2$ & $1$ & $1$ &$2$ & $3$ & $2$ & $3$ & $2$ & $2$ & $2$\\
$S_3$ & $3$ & $2$ & $2$ &$1$ & $4$ & $3$ & $2$  & $2$ & $2$ & $2$
	\end{tabular}}
	\caption{Pairwise Distances}
	\label{metric-pairwisedist}
\end{table}

\paragraph{Input Distribution $\mathcal{D}$ on the Processors' Inputs.}
For $i\in [3]$, let $S_i^1, S_i^2, S_i^3$ be an arbitrary equi-partition of $S_i$. 
Moreover, let $\pi:S \rightarrow [n]$ be a uniformly random bijection. Define the sets 
$Y_1^j = \pi\left(\{b_1^*,b_2^*,a\} \cup S_1^j\right)$, $Y_2^j = \pi\left(\{a^*,c^*,b\} \cup S_2^j\right)$ and $Y_3^j = \pi\left(\{b_1^*,b_2^*,c\} \cup S_3^j\right)$, for $j\in [3]$.
%Though the processors are given the renamed points, we will keep referring to the points by their original names, eg. in the definition of $B_i$ later. \textbf{This creates an impression that $Y^j_i$'s form a random equi-partition of the metric space. What we really mean to say is that $\pi$ is a relabeling of the vertices. For example, $Y_1^1$ gets ${b_1^*,b_2^*,a}\cup S_1^1$, but doesn't know which is which, because the names are garbled. I would suggest define a metric space over an appropriate set $S$, different from $[n]$, containing $a^*,b_1^*,$ etc., and let $\pi:S\longrightarrow[n]$ be a random bijection. }
By the constraints on the sizes of $S_1,S_2,S_3$, we have that each $Y_i^j$ has the same size. 
For simplicity of notation, we rename $Y_i^j$ to $Y_{3(i-1)+j}$.
% \textbf{Looks like there is a bug here. Perhaps you mean $Y_{3(j-1)+i}$?}
The $i$-th processor's input is $Y_{\Gamma(i)}$, where $\Gamma: [9]\rightarrow [9]$ is a uniformly random permutation.
Note that neither the processors nor the coordinator know the permutations $\pi$ and $\Gamma$.

\begin{theorem}\label{thm:lb}
Consider any distributed algorithm for the $9$ processor $3$-center problem on $\mathcal{M}(n')$ and input distribution $\mathcal{D}$, in which each processor communicates an $\ell$-sized subset of its input points, and the coordinator outputs $3$ of the received points.
If $\ell \leq n'/18$, then with probability at least $1.4\cdot 10^{-4}$, the output is no better than a $4$-approximation.
\end{theorem}

Here, although the probability with which the coordinator fails to outputs a better-than-$4$-approximation is only $1.4\cdot 10^{-4}$, it can be \emph{amplified} to $1-\varepsilon$, for any $\varepsilon > 0$.
We discuss the amplification result before presenting the proof of the above theorem.
\begin{theorem}
Let $\epsilon > 0$, $\beta = 1-1.4\cdot 10^{-4}$ and $\alpha = \left.\left\lceil \frac{100}{91}\cdot \log \left(\frac{1}{\varepsilon}\right) \middle/ \log\left(\frac{1}{\beta}\right) \right\rceil\right.$.
Consider any distributed algorithm for the $9$ processor $3\alpha$-center problem, in which each processor communicates an $\ell$-sized subset of its input points, and the coordinator outputs $3$ of the received points.
There exists a metric space and a distribution on input points, where each processor receives $(n'+3)\alpha$ points, such that if  $\ell \leq n'\alpha/1800$, then with probability at least $1-\epsilon$, the output is no better than a $4$-approximation.
\end{theorem}
\begin{proof}
The underlying metric space consists of $\alpha$ disjoint copies of $\mathcal{M}(n')$ separated by an arbitrarily large distance from one another. 
Each processor receives the corresponding set of points from each copy, as in the description of $\mathcal{D}$.

First, note that for any processor, there are at most $\alpha/100$ copies from which more than $n'/18$ points  are communicated. 
By an application of the union bound, we can infer that if each processor communicates at most $n'\alpha/1800$ points to the coordinator, then there are $\left(1-\frac{9}{100}\right)\cdot \alpha$ copies from which no processor sends more than $n'/18$ points.
Theorem~\ref{thm:lb} implies that the coordinator outputs an exact $4$-approximation with probability at least $1-\beta$ on each of at least $91\alpha/100$ independent copies.
Using the independence between the copies further, we can conclude that the coordinator's output fails to be any better than a $4$-approximation with probability at least $1-\beta^{91\alpha/100} \geq 1 - \varepsilon$, which follows from the inequality
$91\alpha/100 \geq \left.\log \left(\frac{1}{\varepsilon}\right) \middle/ \log \frac{1}{\beta}\right.$.
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:lb}]
For $i\in [9]$, define $B_i$ to be the event that the $i$-th processor communicates a point in $\pi(\{a^*,b_1^*,b_2^*,c^*,a,b,c\})$.
Moreover, define the event $G = \cap_{i=1}^9 B_i^c$, where $B_i^c$ is the complement of $B_i$.
First, we claim that $\Pr[B_i] \leq \ell/n'$. 
Indeed, this is true since all points in each processor's input are equidistant and the labels of the input points have been randomly permuted. 
This claim in conjunction with the union bound implies that $\Pr[G] \geq 1-\frac{9\ell}{n'}$.

We proceed to show that there exists three processors, say $1,2$ and $3$, such that for every fixing of the permutation $\Gamma$, the probability conditioned on $G$ that the coordinator's output is a subset of the points received from processors $1,2,3$ is at least $\frac{1}{\binom{9}{3}}$.
For every $i\in [9]$, let $M_i$ be the set of points communicated by the $i$-th processor. 
Define $M = \cup_{i=1}^9 M_i$, and denote by $O$ the set of output points.
In addition, let $E_{\gamma}$ be the event that $\Gamma = \gamma$.
We now define a function $p$ on subsets $I = \{i_1,i_2,i_3\} \subset [9]$ and  permutations $\gamma$ such that $p(I,\gamma) = \Pr[O \subseteq (M_{i_1} \cup M_{i_2} \cup M_{i_3}) \mid G,E_{\gamma}]$.
For every fixing of $\gamma$, since all points in $O$ are chosen from at most three processors, we can say that $\sum_{I\subset [9]: |I|=3} p(I,\gamma) \geq 1$.
Moreover, we have that $p(I,\gamma) = p(I,\gamma')$ for every distinct $\gamma,\gamma'$.
This follows from symmetry and the fact that $\pi$ is a uniformly random bijection.
Let $p^*$ be the largest value of $p$ for any fixing of $\gamma$, and we can assume without loss of generality $p^*$ is achieved for processors $I = \{1,2,3\}$.
As the number of subsets of $[9]$ of size $3$ is $\binom{9}{3}$, we can conclude that $p^* \geq \frac{1}{\binom{9}{3}}$.

Let $E_O$ be the event that $O \subseteq \pi(S_1)$ or $O \subseteq \pi(S_3)$. Conditioned on $E_O$, cost of the output is $4$. 
We now have that $\Pr[E_O] \geq \Pr[G] \cdot \Pr[E_O|G]$.
Using facts $S_1 \subset Y_1 \cup Y_2 \cup Y_3$ and $S_3 \subset Y_7 \cup Y_8 \cup Y_9$, we have 
\begin{align*}
\Pr[E_O\mid G] \geq \Pr[\Gamma(\{1,2,3\}) = \{1,2,3\}] \cdot p^* + \Pr[\Gamma(\{7,8,9\}) = \{1,2,3\}] \cdot p^*  \geq 2 \cdot \frac{3! \cdot 6!}{9!} \cdot \frac{1}{\binom{9}{3}}.
\end{align*}
Since $\Pr[G] \geq 1-\frac{9\ell}{n'}$ and $\ell \leq n'/18$, we get that $\Pr[E_O] \geq 1.4\cdot 10^{-4}$, as desired.
\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "supplementary"
%%% End:


==> lb-proof2.tex <==
\section{Distributed $k$-Center Lower Bound: Take 2}

In this section we present the formal details of the lower bound discussed in Section~4 of the main paper. 
For a natural number $n$, $[n]$ denotes the set $\{1,2,\ldots,n\}$.
%\paragraph{The Communication Model $\mathrm{PSim}$.} TODO: define the model using notation from previous sections.
\paragraph{The metric space $\mathcal{M}(n')$.} 
The point set of this metric space on $n = 9n'+7$ points is given by 
\[S := \{a^*,b_1^*,b_2^*,c^*,a,b,c\} \cup S_1 \cup S_2 \cup S_3,\]
where $|S_1| = |S_2| = |S_3| = 3n'$.
Note that $S_1,S_2,S_3$ are pairwise disjoint and are also disjoint from $\{a^*,b_1^*,b_2^*,c^*,a,b,c\}$. We will call the points $\{a^*,b_1^*,b_2^*,c^*,a,b,c\}$ \textit{critical}. The metric $d:S\times S\longrightarrow\mathbb{R}$ is the shortest-path-length metric induced by the graph shown in Figure \ref{metric} (where $x$ is not a point in $S$ but is only used to define the pairwise distances). The pairwise distances are given in \Cref{metric-pairwisedist}.
Note that if the table entry $i,j$ is indexed by sets, then the entry corresponds to the distance between distinct points in the sets. The following observation can be verified by a case-by-case analysis.

\begin{observation}\label{obs_lb_opt}
The sets $\{a^*,b_1^*,c^*\}$ and $\{a^*,b_2^*,c^*\}$ are the only optimum solutions of the $3$-center problem on $\mathcal{M}(n')$ and they have unit clustering cost. The clustering cost of any subset of $S_1$ is $4$ due to point $c$. Similarly, the clustering cost of any subset of $S_3$ is $4$ due to point $a$.
\end{observation}


\begin{figure}[h]
    \centering{\includegraphics[width=.4\textwidth]{metric1.pdf}}
    \caption{\footnotesize The underlying metric for $n'=2$}
    \label{metric}
\end{figure}
% \textbf{Need to mention that x is not a point in the metric space.}
\begin{table}[htp]
	\ra{1.5}
	\centering
	\adjustbox{max width = \textwidth}{
		\begin{tabular}{@{}c|ccccccccccc@{}}
			 & $a^*$ & $b_1^*$ & $b_2^*$ & $c^*$ & $a$ & $b$ & $c$  & $S_1$ & $S_2$ & $S_3$\\ 
			 \toprule
$a^*$& $0$ & $1$& $1$ &$2$ & $1$ & $2$ & $3$ & $1$ & $2$ & $3$\\
$b_1^*$ & $1$ & $0$ & $2$ &$1$ & $2$ & $1$ & $2$  & $2$ & $1$ & $2$ \\
$b_2^*$ & $1$ & $2$ &$0$ &$1$ & $2$ & $1$ & $2$ & $2$ & $1$ & $2$ \\
$c^*$ & $2$ & $1$ & $1$ &$0$ & $3$ & $2$ & $1$  & $3$ & $2$ & $1$ \\
$a$ & $1$ & $2$ & $2$ &$3$ & $0$ & $3$ & $4$  & $2$ & $3$ & $4$ \\
$b$ & $2$ & $1$ & $1$ &$2$ & $3$ & $0$ & $3$ & $3$ & $2$ & $3$ \\
$c$ & $3$ & $2$ & $2$ &$1$ & $4$ & $3$ & $0$  & $4$ & $3$ & $2$ \\
$S_1$ & $1$ & $2$ & $2$ &$3$ & $2$ & $3$ & $4$ & $2$ & $2$ & $2$ \\
$S_2$ & $2$ & $1$ & $1$ &$2$ & $3$ & $2$ & $3$ & $2$ & $2$ & $2$\\
$S_3$ & $3$ & $2$ & $2$ &$1$ & $4$ & $3$ & $2$  & $2$ & $2$ & $2$
	\end{tabular}}
	\caption{Pairwise Distances}
	\label{metric-pairwisedist}
\end{table}

\paragraph{Input Distribution $\mathcal{D}$ on the Processors' Inputs.}
For $i\in [3]$, let $S_i^1, S_i^2, S_i^3$ be an arbitrary equi-partition of $S_i$ (and therefore, $|S_i^j|=n'$ for all $i,j$). 
%Moreover, let $\pi:S \rightarrow [n]$ be a uniformly random bijection. 
Define the sets 
$Y_1^j = \{b_1^*,b_2^*,a\} \cup S_1^j$, $Y_2^j = \{a^*,c^*,b\} \cup S_2^j$ and $Y_3^j = \{b_1^*,b_2^*,c\} \cup S_3^j$, for $j\in [3]$.
%Though the processors are given the renamed points, we will keep referring to the points by their original names, eg. in the definition of $B_i$ later. \textbf{This creates an impression that $Y^j_i$'s form a random equi-partition of the metric space. What we really mean to say is that $\pi$ is a relabeling of the vertices. For example, $Y_1^1$ gets ${b_1^*,b_2^*,a}\cup S_1^1$, but doesn't know which is which, because the names are garbled. I would suggest define a metric space over an appropriate set $S$, different from $[n]$, containing $a^*,b_1^*,$ etc., and let $\pi:S\longrightarrow[n]$ be a random bijection. }
Observe that each $Y_i^j$ contains exactly $n'+3$ points separated pairwise by distance $2$, and moreover, $3$ of the $n'+3$ points are critical.
%For simplicity of notation, we rename $Y_i^j$ to $Y_{3(i-1)+j}$.
We assign the sets $Y_i^j$ randomly to the nine processors after a random relabeling. Formally, we pick a uniformly random bijection $\pi:S\longrightarrow[n]$ as the relabeling and another uniformly random bijection $\Gamma:[3]\times[3]\longrightarrow[9]$, independent of $\pi$, as the assignment. We assign the set $\pi(Y_i^j)$ to processor $\Gamma(i,j)$ for every $i,j$. When a processor or the coordinator queries the distance between $p$ and $q$ where $p,q\in[n]$, it gets $d(\pi^{-1}(p),\pi^{-1}(q))$ as an answer.
%The $i$-th processor's input is $Y_{\Gamma(i)}$, where $\Gamma: [9]\rightarrow [9]$ is a uniformly random permutation.
Note that neither the processors nor the coordinator know $\pi$ or $\Gamma$.

\begin{theorem}\label{thm:lb}
Consider any distributed algorithm for the $9$ processor $3$-center problem on $\mathcal{M}(n')$ and input distribution $\mathcal{D}$, in which each processor communicates an $\ell$-sized subset of its input points, and the coordinator outputs $3$ of the received points.
If $\ell \leq n'/54$, then with probability at least $1/84$, the output is no better than a $4$-approximation.
\end{theorem}

Here, although the probability with which the coordinator fails to outputs a better-than-$4$-approximation is only $1/84$, it can be \emph{amplified} to $1-\varepsilon$, for any $\varepsilon > 0$.
We discuss the amplification result before presenting the proof of the above theorem.
\begin{theorem}
Let $\epsilon > 0$, $\beta = 1-1.4\cdot 10^{-4}$ and $\alpha = \left.\left\lceil \frac{100}{91}\cdot \log \left(\frac{1}{\varepsilon}\right) \middle/ \log\left(\frac{1}{\beta}\right) \right\rceil\right.$.
Consider any distributed algorithm for the $9$ processor $3\alpha$-center problem, in which each processor communicates an $\ell$-sized subset of its input points, and the coordinator outputs $3$ of the received points.
There exists a metric space and a distribution on input points, where each processor receives $(n'+3)\alpha$ points, such that if  $\ell \leq n'\alpha/1800$, then with probability at least $1-\epsilon$, the output is no better than a $4$-approximation.
\end{theorem}
\begin{proof}
The underlying metric space consists of $\alpha$ disjoint copies of $\mathcal{M}(n')$ separated by an arbitrarily large distance from one another. 
The point set of each copy is distributed independently to the nine processors as described earlier. Observation \ref{obs_lb_opt} implies that the optimum set of $3\alpha$ centers has unit cost. Also, in order to get a better than $4$-approximation, the coordinator must output a better than $4$-approximate solution from every copy. We prove that this is unlikely.
%Each processor receives the corresponding set of points from each copy, as in the description of $\mathcal{D}$.

Since each processor communicates at most $n'\alpha/1800$ points to the coordinator, for any processor there are at most $\alpha/100$ copies from which the it sends more than $n'/18$ points. 
Thus, there are $\left(1-\frac{9}{100}\right)\cdot \alpha=91\alpha/100$ copies from which none of the $9$ processors sends more than $n'/18$ points.
Theorem~\ref{thm:lb} implies that the coordinator's output from any of these $91\alpha/100$ copies is no better than a $4$-approximation with probability at least $1-\beta$.
Using the independence between the copies further, we can conclude that the coordinator's output fails to be any better than a $4$-approximation with probability at least $1-\beta^{91\alpha/100} \geq 1 - \varepsilon$, which follows from the inequality
$91\alpha/100 \geq \left.\log \left(\frac{1}{\varepsilon}\right) \middle/ \log \frac{1}{\beta}\right.$.
\end{proof}

\begin{proof}[\textbf{Proof of Theorem~\ref{thm:lb}}]
Consider any one of the nine processors. It gets the set $\pi(Y_i^j)$ for a uniformly random $(i,j)\in[3]\times[3]$. Furthermore, since $\pi$ is a uniformly random labeling and points in $Y_i^j$ are pairwise equidistant, the processor is neither able to identify the three critical points in its input, nor does it get any information about $(i,j)$. Formally,

\begin{observation}\label{obs_info}
Conditioned on the set of labels that the processor receives, all subsets of three labels are equally likely to be the set of labels of the three critical points, and independently, the processor is equally likely to have received $Y_i^j$ for all $(i,j)$.
\end{observation}

The first consequence of the above observation is that the probability that at least one of the three critical points appears in the set of at most $\ell$ points the processor communicates is at most $3\ell/|Y_i^j|=3\ell/(n'+3)\leq3\ell/n'$. For a given processor $r\in[9]$, let $O_r$ be the set of points it sends to the coordinator, and define $B_r$ to be the event that $O_r$ contains a critical point. Then $\Pr[B_r]\leq3\ell/n'$. Next, define $G$ to be the event that no processor sends a critical point to the corrdinator, that is, $G = \cap_{r=1}^9 B_r^c$, where $B_r^c$ is the complement of $B_r$. Then by the union bound, $\Pr[G] \geq 1-9\cdot\frac{3\ell}{n'}\geq 1/2$, because $\ell\leq n'/54$.

The second consequence of Observation \ref{obs_info} is that the sets $O_r$ are all independent of the random assignment $\Gamma$, even conditional on $G$. Therefore the coordinator fails to get any information about $\Gamma$ from the nine sets $O_1,\ldots,O_9$ it receives. Formally, 
\begin{observation}\label{obs_gamma_info}
Conditioned on $O_1,\ldots,O_9$ and also on $G$, the bijection $\Gamma$ is equally likely to be any of the $9!$ bijections from $[3]\times[3]$ to $[9]$.
\end{observation}
Suppose the coordinator outputs $O$, a set of three points, on receiving $O_1,\ldots,O_9$. Then $O\subseteq O_{r_1}\cup O_{r_2}\cup O_{r_3}$ for some $r_1,r_2,r_3\in[9]$. Define $G'$ to be the event that $\{r_1,r_2,r_3\}=\Gamma(\{(1,1),(1,2),(1,3)\})$ or $\{r_1,r_2,r_3\}=\Gamma(\{(3,1),(3,2),(3,3)\})$. In words, $G'$ is the event that the coordinator's output is contained
%in $\{S_1\cup\{a\}\}$ or in $\{S_3\cup\{c\}\}$,
in $Y_1^1\cup Y_1^2\cup Y_1^3$ or in $Y_3^1\cup Y_3^2\cup Y_3^3$.
Note that the event $G'\cap G$ implies that the coordinator's output is contained
in $S_1^1\cup S_1^2\cup S_1^3=S_1$ or in $S_3^1\cup S_3^2\cup S_3^3=S_3$. Therefore, by Observation \ref{obs_lb_opt}, event $G'\cap G$ implies that the coordinator fails to output a better than $4$-approximation. We are now left to bound $\Pr[G'\cap G]$ from below.

By Observation \ref{obs_gamma_info} and some elementary combinatorics,
%\[\Pr\left[\{r_1,r_2,r_3\}=\Gamma(\{(1,1),(1,2),(1,3)\})\right]=\Pr[\{r_1,r_2,r_3\}=\Gamma(\{(3,1),(3,2),(3,3)\})]=\frac{3!\cdot6!}{9!}=1/82\text{,}\]
\[\Pr\left[\{r_1,r_2,r_3\}=\Gamma(\{1\}\times\{1,2,3\}\})\mid G\right]=\Pr[\{r_1,r_2,r_3\}=\Gamma(\{3\}\times\{1,2,3\}\})\mid G]=\frac{3!\cdot6!}{9!}=\frac{1}{84}\text{,}\]
and therefore, $\Pr[G'\mid G]=1/42$. Thus,
\[\Pr[G'\cap G]=\Pr[G'\mid G]\cdot\Pr[G]\geq\frac{1}{42}\cdot\frac{1}{2}=\frac{1}{84}\text{,}\]
which means that the coordinator fails to output a better than $4$-approximation with probability at least $1/84$, as required.
\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "supplementary"
%%% End:

